PEAS: A Strategy for Crafting Transferable Adversarial Examples

Black box attacks, where adversaries have limited knowledge of the target model, pose a significant threat to machine learning systems. Adversarial examples generated with a substitute model often suffer from limited transferability to the target model. While recent work explores ranking perturbations for improved success rates, these methods see only modest gains. We propose a novel strategy called PEAS that can boost the transferability of existing black box attacks. PEAS leverages the insight that samples which are perceptually equivalent exhibit significant variability in their adversarial transferability. Our approach first generates a set of images from an initial sample via subtle augmentations. We then evaluate the transferability of adversarial perturbations on these images using a set of substitute models. Finally, the most transferable adversarial example is selected and used for the attack. Our experiments show that PEAS can double the performance of existing attacks, achieving a 2.5x improvement in attack success rates on average over current ranking methods. We thoroughly evaluate PEAS on ImageNet and CIFAR-10, analyze hyperparameter impacts, and provide an ablation study to isolate each component's importance.

==> Algorithms/inference_with_AE.tex <==
\label{alg:inference_ae}
\begin{algorithm}
	\caption{BTD detection with AE ($E$, $x_0$, $d$) } 
	\begin{algorithmic}[1]
        \State $x_{0}' = E(x_0)$
        \State $x_d = Backward-Diffusion(x_{0}, T=d)$
        \State $x_{d}' = E(x_{d})$
        \State $score = \frac{1}{W\times H} \sum_{i=1}^{W\times H} (x_{0}'(i) - x_{d}'(i))^2$
	\end{algorithmic} 
\end{algorithm}

==> Algorithms/sampling.tex <==
\label{alg:sampling}
\begin{algorithm}
	\caption{Backward-Diffusion process($\epsilon$, $T$) } 
	\begin{algorithmic}[1]
         \State $x_t = \epsilon$ 
        \For {$t = T,\ldots, 1$}
                \State $z \sim \mathcal{N}(0, I)$ If $t > 1$, Else $z=0$ 
                \State $\Bar{\epsilon} = \epsilon_\theta(x_t, t)$
                \State $\Bar{\mu} = \frac{1}{\sqrt{\alpha_t}}\big(x_t - \frac{1-\alpha_t}{\sqrt{1-\bar{\alpha_t}}}\Bar{\epsilon}\big)$
                \State $x_{t-1} = \bar{\mu} +\sigma_t\cdot z$
    
        \EndFor
        \State Return $x_0$
	\end{algorithmic} 
	
\end{algorithm}

==> Tables/FP_TP.tex <==
\begin{table*}[ht]
    \centering
    
    \caption{Baselines comparison: TPR@FPR10 and FPR@TPR90 results. Bold results are the best and underlined are the second best. CT-GAN is annotated as CT-G}\label{tab:new_results}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{crrrrrr|cccccc}
    
    \multicolumn{1}{l}{} & \multicolumn{6}{c}{TPR@FPR10 $\uparrow$}                                                                             & \multicolumn{6}{c}{FPR@TPR90 $\downarrow$}                                                        \\ \hline\hline
                         & \multicolumn{3}{c}{Injection}                                          & \multicolumn{3}{c|}{Removal}                          & \multicolumn{3}{c}{Injection}                                & \multicolumn{3}{c}{Removal}           \\ \hline
                         & \multicolumn{1}{c}{MRI} & \multicolumn{2}{c|}{CT}                                & \multicolumn{1}{c}{MRI} & \multicolumn{2}{c|}{CT}              & MRI      & \multicolumn{2}{c|}{CT}                           & MRI      & \multicolumn{2}{c}{CT}     \\ \hline
                         & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{CT-G} & \multicolumn{1}{c|}{SD}                   & \multicolumn{1}{c}{SD} & \multicolumn{1}{c}{CT-G} & \multicolumn{1}{c|}{SD} & SD      & CT-G      & \multicolumn{1}{c|}{SD}                   & SD      & CT-G      & SD       \\ \hline
    AE                   & 0.36          & 0.02          & \multicolumn{1}{r|}{0.30}         & 0.75          & 0.06          & 0.79            & 0.46 & 0.66 & \multicolumn{1}{c|}{0.43}         & 0.25 & 0.91 & 0.11 \\
    In-Paint AE          & 0.18          & 0.99          & \multicolumn{1}{r|}{0.99}         & 0.16          & 0.26          & 1.00            & 0.93 & 0.07 & \multicolumn{1}{c|}{0.05}         & 0.60 & 0.77 & 0.22     \\
    OC-VAE               & 0.12          & 0.08          & \multicolumn{1}{r|}{0.18}         & 0.19          & 0.07          & 0.09            & 0.83 & 0.66 & \multicolumn{1}{c|}{0.65}         & 0.85 & 0.91 & 0.88     \\
    Unet-AE              & 0.20          & 0.07          & \multicolumn{1}{r|}{0.16}         & 0.43          & 0.09          & 0.25            & 0.73 & 0.91 & \multicolumn{1}{c|}{0.84}         & 0.70 & 0.89 & 0.76     \\
    Splice Buster        & 0.07          & 0.11          & \multicolumn{1}{r|}{0.08}         & 0.09          & 0.10          & 0.13            & 0.83 & 0.92 & \multicolumn{1}{c|}{0.81}         & 0.96 & 0.88 & 0.77     \\
    Splice Radar         & 0.14          & 0.38          & \multicolumn{1}{r|}{0.12}         & 0.28          & 0.22          & 0.27            & 0.87 & 0.69 & \multicolumn{1}{c|}{0.78}         & 0.79 & 0.87 & 0.79     \\
    Satellite ViT        & 0.20          & 0.05          & \multicolumn{1}{r|}{0.14}         & 0.20          & 0.05          & 0.06            & 0.80 & 0.65 & \multicolumn{1}{c|}{0.68}         & 0.80 & 0.91 & 0.87     \\
    OOD DDPM             & 0.00          & 0.00          & \multicolumn{1}{r|}{0.00}         & 0.00          & 0.00          & 0.00            & 0.00 & 0.00 & \multicolumn{1}{c|}{0.00}         & 0.00 & 0.00 & 0.00     \\
    \textbf{BTD} - 32 dim & 0.00          & 0.00          & \multicolumn{1}{r|}{0.00}         & 0.00          & 0.00          & 0.00            & 0.00 & 0.00 & \multicolumn{1}{c|}{0.00}         & 0.00 & 0.00 & 0.00     \\
    \textbf{BTD} - 8 dim  & 0.00          & 0.00          & \multicolumn{1}{r|}{0.00}         & 0.00          & 0.00          & 0.00            & 0.00 & 0.00 & \multicolumn{1}{c|}{0.00}         & 0.00 & 0.00 & 0.00     \\ \hline\hline
    \end{tabular}
    }
    
    \end{table*}


==> Tables/ablation_noise_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[t]
\caption{Ablation Study: The impact forwards diffusion has on tamper detection. Existing methdos perform both forwards and backwards (F\&B) while BTD only performs backwards (B). The rows indicate the number of steps performed in the indicated direction(s) before measuring the residual. Bold values indicate the best result over 0.6 (close to random guessing).}
\label{tab:noise_ablation}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{cr|ccc|ccc|}
\multicolumn{2}{c|}{} & \multicolumn{3}{c|}{Injection} & \multicolumn{3}{c|}{Removal} \\
\multicolumn{2}{c|}{} & MRI & \multicolumn{2}{c|}{CT} & MRI & \multicolumn{2}{c|}{CT} \\
\multicolumn{2}{c|}{} & SD & CT-G & SD & SD & CT-G & SD \\ \hline
 & \textit{F\&B} & 0.7279 & 0.6839 & 0.7375 & 0.8408 & 0.4828 & 0.6626 \\
\multirow{-2}{*}{1} & \cellcolor[HTML]{EFEFEF}\textit{B} & \cellcolor[HTML]{EFEFEF}\textbf{0.9862} & \cellcolor[HTML]{EFEFEF}\textbf{0.8056} & \cellcolor[HTML]{EFEFEF}\textbf{0.9082} & \cellcolor[HTML]{EFEFEF}\textbf{0.9838} & \cellcolor[HTML]{EFEFEF}0.5524 & \cellcolor[HTML]{EFEFEF}\textbf{0.8607} \\ \hline
 & \textit{F\&B} & 0.5063 & 0.6502 & 0.6982 & 0.6755 & 0.4995 & 0.6086 \\
\multirow{-2}{*}{10} & \cellcolor[HTML]{EFEFEF}\textit{B} & \cellcolor[HTML]{EFEFEF}0.5873 & \cellcolor[HTML]{EFEFEF}0.6405 & \cellcolor[HTML]{EFEFEF}0.6909 & \cellcolor[HTML]{EFEFEF}0.6909 & \cellcolor[HTML]{EFEFEF}0.5061 & \cellcolor[HTML]{EFEFEF}0.6195 \\ \hline
 & \textit{F\&B} & 0.4047 & 0.6385 & 0.7062 & 0.6183 & 0.5059 & 0.6089 \\
\multirow{-2}{*}{50} & \cellcolor[HTML]{EFEFEF}\textit{B} & \cellcolor[HTML]{EFEFEF}0.4152 & \cellcolor[HTML]{EFEFEF}0.6130 & \cellcolor[HTML]{EFEFEF}0.6849 & \cellcolor[HTML]{EFEFEF}0.6058 & \cellcolor[HTML]{EFEFEF}0.5041 & \cellcolor[HTML]{EFEFEF}0.6081 \\ \hline
 & \textit{F\&B} & 0.3995 & 0.6331 & 0.7076 & 0.6025 & 0.4952 & 0.6064 \\
\multirow{-2}{*}{100} & \cellcolor[HTML]{EFEFEF}\textit{B} & \cellcolor[HTML]{EFEFEF}0.4015 & \cellcolor[HTML]{EFEFEF}0.5889 & \cellcolor[HTML]{EFEFEF}0.6895 & \cellcolor[HTML]{EFEFEF}0.5953 & \cellcolor[HTML]{EFEFEF}0.4974 & \cellcolor[HTML]{EFEFEF}0.5980 \\ \hline
 & \textit{F\&B} & 0.4266 & 0.6363 & 0.7231 & 0.6002 & 0.4930 & 0.5911 \\
\multirow{-2}{*}{200} & \cellcolor[HTML]{EFEFEF}\textit{B} & \cellcolor[HTML]{EFEFEF}0.4339 & \cellcolor[HTML]{EFEFEF}0.5685 & \cellcolor[HTML]{EFEFEF}0.6928 & \cellcolor[HTML]{EFEFEF}0.5942 & \cellcolor[HTML]{EFEFEF}0.4838 & \cellcolor[HTML]{EFEFEF}0.5754 \\ \hline
\end{tabular}%
%}
\end{table}

==> Tables/baselines_comparison.tex <==
\def\arraystretch{1.15}%  1 is the default, change whatever you need
\setlength\tabcolsep{.25em}
\begin{table*}[h]
\centering
\resizebox{!}{0.16\textwidth}{
\begin{tabular}{ccccc|cccc}
\hline\hline
\multicolumn{5}{c|}{AUC $\uparrow$}                                                                                                                                                                                 & \multicolumn{4}{c}{EER $\downarrow$}                                                                                                                                          \\ \hline
\multicolumn{1}{l}{} & \multicolumn{2}{c}{Stable Difffusion}                                                                         & \multicolumn{2}{c|}{CT-GAN}                                                  & \multicolumn{2}{c}{Stable Diffusion}                                                                           & \multicolumn{2}{c}{CT-GAN}                                   \\ \hline
                     & MRI-Remove                                 & \multicolumn{1}{c|}{CT-Remove}                                   & CT-Inject                                   & \multicolumn{1}{l|}{CT-Remove} & MRI-Remove                                  & \multicolumn{1}{c|}{CT-Remove}                                   & CT-Inject                                   & CT-Remove      \\ \hline
AE                   & \underline{91.3$\pm$0.49} & \multicolumn{1}{c|}{\underline{83.95$\pm$1.26}} & 58.6$\pm$1.52                               & 46.39$\pm$1.3                  & \underline{18.70$\pm$1.03} & \multicolumn{1}{c|}{\underline{23.21$\pm$2.09}} & 44.59$\pm$1.38                              & \textbf{53$\pm$1.7}     \\
In-Paint AE          & 66.89$\pm$0.85                             & \multicolumn{1}{c|}{56.08$\pm$2.67}                              & \underline{79.83$\pm$1.36} & 39.65$\pm$2.20                 & 33.91$\pm$0.85                              & \multicolumn{1}{c|}{48.05$\pm$2.19}                              & \underline{25.56$\pm$1.28} & 55.72$\pm2.71$ \\
OC-VAE               & 60.11$\pm$0.53                             & \multicolumn{1}{c|}{52.94$\pm$1.9}                               & 60.56$\pm$1.79                              & 47.27$\pm$1.97                 & 45.14$\pm$1.04                              & \multicolumn{1}{c|}{49.05$\pm$2.3}                               & 42.85$\pm$1.70                              & \underline{52.75$\pm$1.97} \\
Unet-AE              & 72.88$\pm$0.51                             & \multicolumn{1}{c|}{81.79$\pm$1.54}                              & 48.61$\pm$1.94                              & 47.54$\pm$1.58                 & 34.76$\pm$0.86                              & \multicolumn{1}{c|}{23.40$\pm$2.09}                              & 50.88$\pm$1.80                              & 52.46$\pm$1.58 \\
Splice Buster        & 47.79$\pm$1.80                             & \multicolumn{1}{c|}{59.18$\pm$2.49}                              & 48.58$\pm$1.78                              & 49.89$\pm$2.49                 & 48.63$\pm$1.65                              & \multicolumn{1}{c|}{45.1$\pm$2.57}                               & 50.97$\pm$1.63                              & 52.16$\pm$2.49 \\
Splice Radar         & 69.48$\pm$1.16                             & \multicolumn{1}{c|}{65.82$\pm$2.20}                              & 77.47$\pm$1.59                              & \textbf{60.64$\pm$2.27}                 & 35.21$\pm$1.11                              & \multicolumn{1}{c|}{37.43$\pm$2.36}                              & 28.99$\pm$1.66                              & 42.02$\pm$2.27 \\
Satellite ViT        & 65.32$\pm$0.45                             & \multicolumn{1}{c|}{53.12$\pm$1.04}                              & 78.01$\pm$1.35                              & 47.51$\pm$1.06                 & 38.84$\pm$1.26                              & \multicolumn{1}{c|}{46.34$\pm$1.53}                              & 27.23$\pm$1.32                              & 50.11$\pm$1.06 \\
    BTD (ours)           & \textbf{95.76$\pm$0.09}   & \multicolumn{1}{c|}{\textbf{88.28$\pm$1.40}}    & \textbf{83.38$\pm$1.44}    & \underline{55.03$\pm$1.44}                 & \textbf{6.73$\pm$1.7}      & \multicolumn{1}{c|}{\textbf{18.32$\pm$1.81}}    & \textbf{21.23$\pm$1.32}    & 44.61$\pm$1.44 \\ \hline\hline
\end{tabular}
}
\end{table*}

==> Tables/new_AUC_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[t]
\caption{Baselines comparison: The AUC of BTD compared to the baselines for each of the six attack scenarios. Bold values indicate the best result over 0.6 (close to random guessing).}
\label{tab:main_results}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc|ccc|}
\textit{\textbf{}} & \multicolumn{3}{c|}{Injection} & \multicolumn{3}{c|}{Removal} \\ \cline{2-7} 
 & MRI & \multicolumn{2}{c|}{CT} & MRI & \multicolumn{2}{c|}{CT} \\ \cline{2-7} 
 & SD & CT-GAN & SD & SD & CT-GAN & SD \\ \hline
AE & 0.80 & 0.56 & 0.79 & 0.91 & 0.45 & 0.93 \\
In-Paint AE & 0.52 & 0.80 & 0.76 & 0.65 & 0.60 & 0.56 \\
OC-VAE & 0.54 & 0.62 & 0.68 & 0.58 & 0.48 & 0.52 \\
Unet-AE & 0.63 & 0.46 & 0.71 & 0.73 & 0.48 & 0.92 \\
Splice Buster & 0.48 & 0.49 & 0.54 & 0.46 & 0.50 & 0.59 \\
Splice Radar & 0.55 & 0.73 & 0.61 & 0.62 & 0.57 & 0.65 \\
Satellite ViT & 0.54 & 0.61 & 0.65 & 0.63 & 0.47 & 0.51 \\
OOD DDPM & 0.50 & 0.54 & 0.53 & 0.63 & 0.42 & 0.49 \\
\rowcolor[HTML]{EFEFEF} 
\textbf{BTD} - 32 dim & \textbf{0.99} & \textbf{0.81} & \textbf{0.91} & \textbf{0.98} & 0.55 & 0.86 \\
\rowcolor[HTML]{EFEFEF} 
\textbf{BTD} - 8 dim & 0.93 & 0.69 & 0.87 & 0.93 & 0.52 & \textbf{0.94} \\ \hline
\end{tabular}%
%}
\end{table}

==> Tables/processing.tex <==
\begin{table*}[ht!]
\centering
\caption{Summary of data preprocessing for CT and MRI modalities.}
\label{tab:preprocessing}
\begin{tabular}{c|cc}
\hline
              & CT               & MRI              \\ \hline
Grouping      & None             & Per-patient      \\ \hline
Clipping      & -700 to 2000     & None             \\ \hline
Normalization & [0, 1]           & [0, 1]           \\ \hline

\end{tabular}

\end{table*}


==> Tables/scanner_comparison.tex <==
\begin{table*}[ht]
\centering

\caption{The performance of BTD when applied to images taken from different medical imaging devices.}
\label{Table:Scanners}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccc}
    \begin{tabular}[t]{ccc}
        \multicolumn{3}{c}{SD-CT-Inject}\\
        \hline\hline
        \textit{Scanner} & \textit{AUC} & \textit{EER} \\ \hline
        LightSpeed16 & 0.93 & 0.15 \\
        Sensation 16 & 0.94 & 0.10 \\
        LightSpeed Pro 16 & 0.93 & 0.18 \\
        LightSpeed Ultra & 0.85 & 0.22 \\
        LightSpeed QX & 0.89 & 0.17 \\
        \hline\hline
    \end{tabular}
    &
    \begin{tabular}[t]{ccc}
        \multicolumn{3}{c}{CTGAN-CT-Inject}\\
        \hline\hline
        \textit{Scanner} & \textit{AUC} & \textit{EER} \\ \hline
        LightSpeed16 & 0.75 & 0.28 \\
        Sensation 16 & 0.96 & 0.10 \\
        LightSpeed Pro 16 & 0.90 & 0.18 \\
        LightSpeed Ultra & 0.66 & 0.42 \\
        LightSpeed QX & 0.69 & 0.38 \\
        \hline\hline
    \end{tabular}
    &
    \begin{tabular}[t]{ccc}
        \multicolumn{3}{c}{SD-MRI-Inject}\\
        \hline\hline
        \textit{Scanner} & \textit{AUC} & \textit{EER} \\ \hline
        Avanto & 0.92 & 0.20 \\ 
        Optima MR450w & 1.00 & 0.00 \\ 
        SIGNA HDx & 1.00 & 0.00 \\ 
        Signa HDxt & 1.00 & 0.01 \\ 
        \hline\hline
    \end{tabular}
    \\
    \\

    \begin{tabular}[t]{ccc}
        \multicolumn{3}{c}{SD-CT-Remove}\\
        \hline\hline
        \textit{Scanner} & \textit{AUC} & \textit{EER} \\ \hline
        LightSpeed16 & 0.92 & 0.15 \\ 
        Sensation 16 & 0.93 & 0.14 \\ 
        LightSpeed Ultra & 0.85 & 0.23 \\ 
        LightSpeed QX & 0.78 & 0.28 \\
        \hline\hline
    \end{tabular}
    &
    \begin{tabular}[t]{ccc}
        \multicolumn{3}{c}{CTGAN-CT-Remove}\\
        \hline\hline
        \textit{Scanner} & \textit{AUC} & \textit{EER} \\ \hline
        LightSpeed16 & 0.56 & 0.45 \\
        Sensation 16 & 0.56 & 0.44 \\
        LightSpeed Ultra & 0.58 & 0.44 \\
        LightSpeed QX & 0.52 & 0.48 \\
        \hline\hline
    \end{tabular}
    &
        \begin{tabular}[t]{ccc}
        \multicolumn{3}{c}{SD-MRI-Remove}\\
        \hline\hline
        \textit{Scanner} & \textit{AUC} & \textit{EER} \\ \hline
        Avanto & 0.97 & 0.09 \\ 
        Optima MR450w & 1.00 & 0.02 \\ 
        SIGNA HDx & 1.00 & 0.00 \\ 
        Signa HDxt & 1.00 & 0.00 \\ 
        \hline\hline
    \end{tabular}
\end{tabular}
}

\vspace{-1em}
\end{table*}

